Leveraging Large Vision Language Model For Better Automatic Web GUI Testing

With the rapid development of web technology, more and more software applications have become web-based in the past decades. To ensure software quality and user experience, various techniques have been proposed to automatically test web applications by interacting with their GUIs. To achieve high functional coverage, web GUI testing tools often need to generate high-quality text inputs and interact with the associated GUI elements (e.g., click submit buttons). However, developing a holistic approach that solves both subtasks is challenging because the web GUI context can be complicated and highly dynamic, which makes it hard to process programmatically. The recent development of large vision-language models (LVLM) provides new opportunities to handle these longstanding problems. This paper proposes VETL, the first LVLM-driven end-to-end web testing technique. With LVLM's scene understanding capabilities, VETL can generate valid and meaningful text inputs focusing on the local context, while avoiding the need to extract precise textual attributes. The selection of associated GUI elements is formulated as a visual question-answering problem, allowing LVLM to capture the logical connection between the input box and the relevant element based on visual instructions. Further, the GUI exploration is guided by a multi-armed bandit module employing a curiosity-oriented strategy. Experiments show that VETL effectively explores web state/action spaces and detects bugs. Compared with WebExplor, the state-of-the-art web testing technique, VETL can discover 25% more unique web actions on benchmark websites. Moreover, it can expose functional bugs in top-ranking commercial websites, which the website maintainers have confirmed. Our work makes the first attempt at leveraging LVLM in end-to-end GUI testing, demonstrating promising results in this research direction.

==> table/prompt_template_colored.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{tabular}{c|ll}
\toprule
\textbf{Template} &
  \multicolumn{1}{c|}{\textbf{Input Prompt}} &
  \multicolumn{1}{c}{\textbf{Element Prompt}} \\ \midrule
\begin{tabular}[c]{@{}c@{}}Role Playing\\ $\left \langle \textit{RP}\right \rangle $\end{tabular} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}
  \cellcolor{orange!20}You are working as a web tester and your task is to generate input text for\\ 
  \cellcolor{orange!20}the box on the web page you are viewing.\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}
  \cellcolor{LimeGreen!20}Your task is to   select a button on a webpage that needs to be clicked after filling in \\
  \cellcolor{LimeGreen!20}the input box, in order to submit the filled content and ensure the effectiveness of \\
  \cellcolor{LimeGreen!20}the input box testing.\end{tabular} \\ \midrule
 &
  \multicolumn{2}{c}{\cellcolor{Lavender!20}The web page you are viewing has the title: \{\textit{HTML Title}\}.} \\ 
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Global Context\\ $\left \langle \textit{GC}\right \rangle $\end{tabular}} &
  \multicolumn{2}{c}{{\cellcolor{Lavender!20}\color[HTML]{A6A6A6} e.g. The web   page you are viewing has the title:\{\textit{Splittypie}\}.}} \\ \midrule
 &
  \multicolumn{2}{c}{\cellcolor{Purple!10}This text is placed next to the input box: \{\textit{text of Near Widgets}\}.} \\ 
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Local Context\\ $\left \langle LC\right \rangle $\end{tabular}} &
  \multicolumn{2}{c}{{\cellcolor{Purple!10}\color[HTML]{A6A6A6} e.g.   This text is placed next to the input box: \{\textit{How much? USD}\}}} \\ \midrule
 &
  \multicolumn{1}{l|}{\cellcolor{Yellow!15}1. The type of   this input is \{\textit{type of Input Widget}\}.} &\cellcolor{SpringGreen!20}
   \\
 &
  \multicolumn{1}{l|}{{\cellcolor{Yellow!15}\color[HTML]{A6A6A6} e.g. The type of this   input is \{\textit{number}\}.}} &\cellcolor{SpringGreen!20}
   \\
 &
  \multicolumn{1}{l|}{\cellcolor{Yellow!15}2. This input is about \{\textit{id\ /\ placeholder\ /\ name of Input Widget}\}.} &\cellcolor{SpringGreen!20}
   \\
 &
  \multicolumn{1}{l|}{{\cellcolor{Yellow!15}\color[HTML]{A6A6A6} e.g.   This input is about \{\textit{Amount}\}.}} &
  \multirow{-1}{*}{\cellcolor{SpringGreen!20}The content filled in the input box is \{\textit{Generated Input Text}\}.} \\
 &
  \multicolumn{1}{l|}{\cellcolor{Yellow!15}3. This input can be    \{\textit{value of Input Widget}\}.} &
  {\cellcolor{SpringGreen!20}\color[HTML]{A6A6A6} } \\
 &
  \multicolumn{1}{l|}{{\cellcolor{Yellow!15}\color[HTML]{A6A6A6} /}} &
  {\cellcolor{SpringGreen!20}\color[HTML]{A6A6A6} } \\
 &
  \multicolumn{1}{l|}{\cellcolor{Yellow!15}4. The input have some constraints: \{\textit{Constraint Attributes of Input Widget}\}.} &
  {\cellcolor{SpringGreen!20}\color[HTML]{A6A6A6} } \\
\multirow{-8}{*}{\begin{tabular}[c]{@{}c@{}}Input Widget\\ $\left \langle IW\right \rangle $\end{tabular}} &
  \multicolumn{1}{l|}{{\cellcolor{Yellow!15}\color[HTML]{A6A6A6} e.g. The input have some constraints: \{\textit{The minimum value   is 0}\}}} &
  \multirow{-7}{*}{\cellcolor{SpringGreen!20}{\color[HTML]{A6A6A6} e.g. The content filled in the input box is \{\textit{199}\}.}} \\ \midrule
\begin{tabular}[c]{@{}c@{}}Visual Information\\ $\left \langle \textit{VI}\right \rangle $\end{tabular} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\cellcolor{Apricot!20}You are provided with a screenshot of the webpage you are browsing, where\\ \cellcolor{Apricot!20}the input box to be filled is marked with a \textcolor{red}{red} box.\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}
  \cellcolor{SeaGreen!15}You are provided with a screenshot of the webpage you are browsing, where the \\ 
  \cellcolor{SeaGreen!15}input box to be filled is marked with a red box and the buttons to be selected are\\ 
  \cellcolor{SeaGreen!15}marked with numbers and \textcolor{blue}{blue}  boxes.\end{tabular} \\ \midrule
\begin{tabular}[c]{@{}c@{}}Output Structure\\ $\left \langle \textit{OS}\right \rangle $\end{tabular} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}
  \cellcolor{RedOrange!20}Your job is to provide the appropriate content for the input box. Only return\\ 
  \cellcolor{RedOrange!20}the generated content without any explanation. Use the following format for\\ 
  \cellcolor{RedOrange!20}your answer: Generated Input Text: {[}Answer{]}\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}
  \cellcolor{BlueGreen!20}Your job is to select one of the buttons and return the number associated with the\\ 
  \cellcolor{BlueGreen!20}selected button. Use the following format for your answer: Button: {[}number{]}\end{tabular} \\ \bottomrule
\textbf{\begin{tabular}[c]{@{}c@{}}Vision Prompt\\ Generation\\ Rules\end{tabular}} &
  \multicolumn{1}{c|}{\colorbox{orange!20}{$\left \langle \textit{RP}\right \rangle $}+\colorbox{Lavender!20}{$\left \langle \textit{GC}\right \rangle $}+\colorbox{Purple!10}{$\left \langle LC\right \rangle $}+\colorbox{Yellow!15}{$\left \langle IW\right \rangle $}+\colorbox{Apricot!20}{$\left \langle \textit{VI}\right \rangle $}+\colorbox{RedOrange!20}{$\left \langle \textit{OS}\right \rangle $}} &
  \multicolumn{1}{c}{\colorbox{LimeGreen!20}{$\left \langle \textit{RP}\right \rangle $}+\colorbox{Lavender!20}{$\left \langle \textit{GC}\right \rangle $}+\colorbox{Purple!10}{$\left \langle LC\right \rangle $}+\colorbox{SpringGreen!20}{$\left \langle IW\right \rangle $}+\colorbox{SeaGreen!15}{$\left \langle \textit{VI}\right \rangle $}+\colorbox{BlueGreen!20}{$\left \langle \textit{OS}\right \rangle $}} \\ \bottomrule
\end{tabular}

